Community aware group testing

In this paper, we propose algorithms that leverage a known community structure to make group testing more efficient. We consider a population organized in disjoint communities: each individual participates in a community, and its infection probability depends on the community (s)he participates in. Use cases include families, students who participate in several classes, and workers who share common spaces. Group testing reduces the number of tests needed to identify the infected individuals by pooling diagnostic samples and testing them together. We show that if we design the testing strategy taking into account the community structure, we can significantly reduce the number of tests needed for adaptive and non-adaptive group testing, and can improve the reliability in cases where tests are noisy.

==> Long_noisy.tex <==
%============================================
In this section we will provide further results and some of the details used in \Cref{sec:Noisy-Testing}. As mentioned earlier, we will  focus on the specific $Z$-channel for the noise model,  where positive test output can flip with probability $\znoiseProb$, illustrated in Fig.~\ref{fig_Zchannel}, reproduced below for convenience. The ideas can be extended to other noise models, but for simplicity we analyze this to focus on the important false negative results. 

%\begin{figure}[!h]
%	\centering
%	\begin{tikzpicture}
%	\node at (-0.8,0.6) {$Y_\tau$}; \node at (2.8,0.6) {$\hat{Y}_\tau$}; 
%	\draw[->,>=stealth] (0,0)--(2,0); \node[below] at (1,0) {$1-\znoiseProb$}; \node[left] at (0,0) {$1$}; \node[right] at (2,0) {$1$};
%	\draw[-stealth,red] (0,0)--(2,1.2); \node[left] at (1.5,0.5) {$\znoiseProb$}; 
%	\draw[-stealth] (0,1.2)--(2,1.2);   \node[left] at (0,1.2) {$0$}; \node[right] at (2,1.2) {$0$};
%	\end{tikzpicture}
%\caption{Z-channel noise.}
%\end{figure}


%\subsection{Reliability of testing without community structure} \label{subsec:NoisyTestNoComm}
We briefly analyze the performance of some testing strategies which use the traditional group testing methods, without taking into account the community structure. The goal is then to compare these with the methods that utilize the community structure, adapting algorithms considered in \Cref{section-algorithm} for the noise-free (or noiseless) case to the case of testing with noise.

\subsection{Repetition testing}
In the presence of noisy tests, the simplest way to correct for noisy tests is to test each item repeatedly, saying $\ell$ times. 
In such a strategy, the testing matrix is composed of $\ell$ identity matrix $I_{n}$, i.e. $\testmatrix=[I_n,\cdots,I_n]^T$. 
It is well-known that a length-$\ell$ repetition code can correct up to $\frac{\ell-1}{2}$ noise-related flips. 
For each item $i\in\mathcal{N}$, the decision rule is given as follows,
\begin{equation}
\label{eq:RepTestCond}
\hat{\defectValue}_i=
\begin{cases}
0,&\text{if } |\{t\in\mathcal{C}_i: \hat{y}_t=0\}|>(1+\delta)\znoiseProb\ell  \\
1,&\text{if }|\{t\in\mathcal{C}_i: \hat{y}_t=1\}|\geq \ell-(1+\delta)\znoiseProb\ell,
\end{cases}
\end{equation}
where tunable parameter  $\delta\geq 0$ and $\mathcal{C}_i= \{i,i+n,\cdots,i+(\ell-1)n\}$, $i\in\mathcal{N}$ is the test set of item $i$. 
\begin{lemma}
\label{lem:RepTest}
Using the threshold decoding rule given in \eqref{eq:RepTestCond}, 
the probability of false negative is bounded as 
\begin{equation}
\label{eq:lem:RepTest}
P(\text{FN}|\text{Repetition}) \leq e^{-2\frac{T}{n}(\znoiseProb\delta)^2},
\end{equation}
\end{lemma}
\noindent where $\nTests$ is the total number of tests for a total population size $\nItems$; also note that there are no false positives in  this due to the $Z$-channel noise model.
\begin{proof}
For any item $\defectValue_i$, the false negative probability is
\begin{align*}
P(\text{FN}|\text{Repetition})&=\Pr(\hat{\defectValue}_i=0|\defectValue_i=1)  \\
&=\sum_{j=(1+\delta)\znoiseProb\ell+1}^{\ell}{\ell \choose j}\znoiseProb^j(1-\znoiseProb)^{\ell-j}  \\
&\leq e^{-2\ell(z\delta)^2} \\
&=e^{-2\frac{T}{n}(z\delta)^2}, 
\end{align*}
where the inequality follows from the Chernoff bound. 
\end{proof}

This simple method can  obtain a small false negative probability, with a large number of tests, which is $\ell$ times the total number of items, $\nTests=\ell \nItems$. 
Next, we consider group testing which could significantly reduce the number of tests, which is analyzed for reliability.


%%%---------------------------------------------------
\subsection{Group testing for noisy tests} \label{app:subsec:noisyGroupTest}
As noted earlier, just as in coding theory, repetition is not as efficient as a coded mechanism, we analyze the performance of group testing (effectively coding), with some redundancy, for noisy tests.
For the analysis we focus on two classes of testing matrix $\testmatrix$, which are studied in literature: Bernoulli designs and constant weight designs \cite[p.10]{GroupTestingMonograph}, which were defined in \Cref{sec:Noisy-Testing} and repeated below for convenience. 
Let $\testmatrixEntry_{t,i}$ be the entries of (random) matrix $\testmatrix$.

\noindent\textbf{Decoder:} 
%Ideally, one would use an optimal decoder for group testing with noise \cite{GroupTestingMonograph}, whose relaxation can be implemented using a linear program (see Section \ref{app:subsec:LPdec} for details). However, such decoders are difficult to analyze (though  we use it for our numerical results). For  simplicity of analysis, we use a threshold-based rule to decode each item individually, described below. 
We use a threshold-based rule (similar to the COMP in \cite{Nonadaptive-1}) to decode each item individually, described below. 
For each $i\in\mathcal{N}$, we identify whether member $i$ is an infected member through the $i$-th column of $\testmatrix$. 
Among all the outputs corresponding to $\tau\in\mathcal{T}$ such that $\testmatrixEntry_{\tau,i}=1$, if the number of ones is larger than some threshold, 
then we say $i$ is an infected member. Otherwise, we say $i$ is non-infected. 
Formally, for a tunable parameter $\delta\geq 0$, we write the decoding rule as: 
\begin{equation}
\hat{\defectValue}_i=
\begin{cases}
0,&\text{if }|\{\tau\in\mathcal{T}: \hat{y}_{\tau}=0,\testmatrixEntry_{\tau,i}=1\}| \\
&\quad >\znoiseProb(1+\delta)\cdot |\{\tau\in\mathcal{T}:\testmatrixEntry_{\tau,i}=1\}| \\
1,&\text{if }|\{\tau\in\mathcal{T}: \hat{y}_{\tau}=1,\testmatrixEntry_{\tau,i}=1\}| \\
&\quad \geq (1-\znoiseProb(1+\delta))\cdot |\{\tau\in\mathcal{T}:\testmatrixEntry_{\tau,i}=1\}|.
\end{cases}  \label{Bernoulli-threshold-decision-rule}
\end{equation}
for each $i\in\mathcal{N}$.  
The Bernoulli and constant-weight testing matrices are defined in \Cref{sec:Noisy-Testing}, and repeated below for convenience,
\begin{itemize}
	\item\textbf{Bernoulli design:} each item is included in each test independently at random with probability $\bernoulliProb$, i.e.
	\begin{equation}
	P(\testmatrixEntry_{t,i}=1)=\bernoulliProb, \forall~i\in\{1,2,\cdots,n\}, t\in\mathcal{T}.   \label{def-Bernoulli}
	\end{equation}
	%	Typically, the parameter $p$ is chosen to scale as $p=\Theta(1/k)$. 
	
	\item \textbf{Constant weight design:} each item is included in $L$ tests, which are chosen uniformly at random, independent from the choices for all other items. 
	In terms of the testing matrix $\testmatrix$, we have independent columns of constant weight. 
	%	Typically, the parameter $L$ is chosen to scale as $L=\Theta(T/k)$.
\end{itemize}

%%%---------------------------------------------------
\subsubsection{Bernoulli testing matrix:} 
The false negative and false positive probabilities with Bernoulli design matrix are bounded as follows.
\begin{lemma}
\label{lem:FNP-Bern}
For the Bernoulli  testing matrix $\testmatrix$ defined in \eqref{def-Bernoulli} and
the threshold decoding rule in \eqref{Bernoulli-threshold-decision-rule}, the probability of false negative is bounded as
\begin{align}
\label{eq:lem:FN-Bern}
P(\text{FN}|\text{Bernoulli}) \leq \left(1-\bernoulliProb+\bernoulliProb e^{-2(\znoiseProb\delta)^2}\right)^{\nTests}.
\end{align}
Similarly, the probability of false positive can be bounded as
\begin{equation}
 \label{eq:lem:FP-Bern}   
 P(\text{FP}|\text{Bernoulli}) \leq \left(1-\bernoulliProb+\bernoulliProb e^{-2((1-\znoiseProb)(1-\bernoulliProb)^k-\znoiseProb\delta)^2}\right)^{\nTests}. 
\end{equation}
\end{lemma}
\begin{proof}
For any infected member $i$, the false negative probability is
\begin{align*}
&P(\text{FN}|\text{Bernoulli}) \nonumber \\
&=\Pr(\hat{\defectValue}_i=0|\defectValue_i=1)  \nonumber \\
&=\sum_{j=1}^{T}{T \choose j}\bernoulliProb^j(1-\bernoulliProb)^{T-j}\left(\sum_{s=\znoiseProb(1+\delta)j}^{j}{j\choose s}\znoiseProb^s(1-\znoiseProb)^{j-s}\right) \nonumber \\
&\leq \sum_{j=0}^{T}{T \choose j}\bernoulliProb^j(1-\bernoulliProb)^{T-j}e^{-2j(\znoiseProb\delta)^2}  \\ %\label{P-Bernoulli-threshold-Chernoff}  \\
&=\left(1-\bernoulliProb+\bernoulliProb e^{-2(\znoiseProb\delta)^2}\right)^{T},  % \label{P-Bernoulli-threshold}
\end{align*}
where the inequality follows from the Chernoff bound. 

Similarly, the false positive probability for any non-infected member $i$ is obtained as follows,  
\begin{align*}
&P(\text{FP}|\text{Bernoulli}) \nonumber \\
&=\Pr(\hat{\defectValue}_i=1|\defectValue_i=0)  \nonumber \\
&=\sum_{j=1}^{T}{T \choose j}\bernoulliProb^j(1-\bernoulliProb)^{T-j}\sum_{s=(1-\znoiseProb(1+\delta))j}^{j}{j\choose s} \cdot \nonumber \\
&~ \left((1-\znoiseProb)(1-(1-\bernoulliProb)^k)\right)^s \left(\znoiseProb(1-(1-\bernoulliProb)^k)+(1-\bernoulliProb)^k\right)^{j-s} \nonumber \\
&\leq \sum_{j=0}^{T}{T \choose j}\bernoulliProb^j(1-\bernoulliProb)^{T-j}e^{-2j(\delta_1(1-\znoiseProb)(1-(1-\bernoulliProb)^k))^2} \\ %\label{P-FP-Bernoulli-threshold-Chernoff}  \\
&= \sum_{j=0}^{T}{T \choose j}\bernoulliProb^j(1-\bernoulliProb)^{T-j}e^{-2j((1-\znoiseProb)(1-\bernoulliProb)^k-\znoiseProb\delta)^2}  \nonumber  \\
&=\left(1-\bernoulliProb+\bernoulliProb e^{-2((1-\znoiseProb)(1-\bernoulliProb)^k-\znoiseProb\delta)^2}\right)^{T},  %\label{P-FP-Bernoulli-threshold}
\end{align*}
where the inequality follow from Chernoff bound and $\delta_1=\frac{1-\znoiseProb(1+\delta)}{(1-\znoiseProb)(1-(1-\bernoulliProb)^k)}-1$.
\end{proof}


%%%---------------------------------------------------
\subsubsection{Constant weight testing matrix}
Replacing Bernoulli testing matrix with the constant weight design in  the following with  the
decision rule in \eqref{Bernoulli-threshold-decision-rule} unchanged. Since the we test $L$ times for each item, the decision rule can be simplified as 
\begin{equation}
\hat{\defectValue}_i=
\begin{cases}
0,&\text{if }|\{t\in\mathcal{T}: \hat{y}_t=0,\testmatrixEntry_{t,i}=1\}|>\znoiseProb(1+\delta)L \\
1,&\text{if }|\{t\in\mathcal{T}: \hat{y}_t=1,\testmatrixEntry_{t,i}=1\}|\geq (1 \!-\! \znoiseProb(1+\delta))L.
\end{cases}  \label{Constant-threshold-decision-rule}
\end{equation}
\begin{lemma}
\label{lem:FNP-CW}
The probability of false negatives is obtained as follows 
\begin{align}
P(\text{FN}|\text{Constant}) &\leq e^{-2L(\znoiseProb\delta)^2}  \label{eq:lem:FN-CW} \\
P(\text{FP}|\text{Constant}) &\leq e^{-2L(\znoiseProb\delta)^2}.  \nonumber 
\end{align}
\end{lemma}
\begin{proof}
The false  negatives for this design can be bounded as follows.
\begin{align}
&P(\text{FN}|\text{Constant}) \nonumber \\
&=\Pr(\hat{\defectValue}_i=0|\defectValue_i=1)  \nonumber \\
&=\Pr(|\{t\in\mathcal{T}: \hat{y}_t=0,\testmatrixEntry_{t,i}=1\}|>\znoiseProb(1+\delta)L\big|\defectValue_i=1)  \nonumber \\
&=\left(\sum_{s=\znoiseProb(1+\delta)L}^{L}{L\choose s}\znoiseProb^s(1-\znoiseProb)^{L-s}\right)  \nonumber \\
&\leq e^{-2L(\znoiseProb\delta)^2},  \label{P-Constant-threshold} 
\end{align}
where \eqref{P-Constant-threshold} follows from the Chernoff bound. 
Similarly the false positive probability can be obtained as follows,
\begin{align}
&P(\text{FP}|\text{Constant})  \nonumber \\
&=\Pr(\hat{\defectValue}_i=1|\defectValue_i=0)  \nonumber \\
&=\Pr(|\{t\in\mathcal{T}: \hat{y}_t=1,\testmatrixEntry_{t,i}=1\}|\geq (1-\znoiseProb(1+\delta))L\big|\defectValue_i=0) \nonumber \\
&=\sum_{\gamma=(1-\znoiseProb(1+\delta))L}^{L}{L \choose \gamma}\left[\frac{{T-L+\gamma \choose L}}{{T \choose L}}\right]^k  \nonumber \\ 
&\qquad\qquad \cdot \sum_{s=(1-\znoiseProb(1+\delta))L}^{\gamma}{\gamma \choose s}(1-\znoiseProb)^s\znoiseProb^{\gamma-s} \nonumber \\
&\leq \sum_{\gamma=(1-\znoiseProb(1+\delta))L}^{L}{L \choose \gamma}\left[\frac{{T-L+\gamma \choose L}}{{T \choose L}}\right]^k \cdot e^{-2L(\znoiseProb\delta)^2} \label{P-FP-Constant-threshold-Chernoff}  \\
%&=(n-k)e^{-\frac{2\left((1-\znoiseProb)\left(1-\frac{L}{T}\right)^k-\znoiseProb\delta\right)^2 T}{k}},   \label{P-FP-Constant-threshold}  \\
&\leq e^{-2L(\znoiseProb\delta)^2},   \label{P-FP-Constant-threshold}
\end{align}
where \eqref{P-FP-Constant-threshold-Chernoff} follows from Chernoff bound. 
\end{proof}


\subsection{Linear Programming decoding}
\label{app:subsec:LPdec}
For a given testing matrix $\testmatrix$, instead of the above decoding algorithm, one may use a linear programming (LP) decoding scheme~\cite[\S3.2]{GroupTestingMonograph},
by solving the following optimization problem: 
\begin{align*}
\min_{\bm{\defectValue},\xi} ~&~ \sum_{i=1}^{\nItems}\defectValue_i+\zeta\sum_{t=1}^{\nTests_2}\xi_i  \\
\text{subject to} ~&~ \sum_{i=1}^{\nItems}\testmatrixEntry_{t,i} \defectValue_i=\xi_t, \text{ when }\hat{y}_t=0 \\
&~ \sum_{i=1}^{\nItems}\testmatrixEntry_{t,i}\defectValue_i\geq 1, \text{ when }\hat{y}_t=1 \\
%	&~ \xi_t=0, \text{ when }\hat{y}=1 \\
&~ 0\leq \xi_t\leq k  \\
&~ 0\leq \defectValue_i\leq 1.     %\\&~ \sum_{i=1}^nu_i=k.
\end{align*}
The LP is a relaxation of the corresponding integer programming by relaxing $\defectValue_i\in\{0,1\}$ to $\defectValue_i\in[0,1]$. 
The solution of $\bm{\defectValue}$ represents an estimate of the infection indicator vector, and we will round each $\defectValue_i$ to its nearest integer from $\{0,1\}$. 

The slack variable $\xi_i$ has the following intuition: i) $\xi_i=0$ if test $\tau$ is positive or truly negative (no error); ii) $\xi_i=$ number of infected members in test $\tau$, if the test is a false negative. 
The parameter $\zeta$ controls the tradeoff between declaring a small number of infected members (sparsity) and the a smaller number of $Z$-channel noise-related flips happen (most slack variables being zero).

Although an LP decoder is an option, we observed no significant benefits when using it in our experiments. 
So, we preferred the much faster COMP decoder of~\eqref{Bernoulli-threshold-decision-rule}.



\subsection{Proof of \Cref{lemma-exponential-FNprob-noisy}}
\label{app:lemma-exponential-FNprob-noisy}
%We want to compare the two-stage algorithm taking community structure into account against traditional group testing that again uses the same mechanism for redundancy but does not take into account the community structure. 
Let $Q$ denotes the false negative probability for each infected member in the traditional group testing. 
In the two-stage algorithm, we use $Q_1$, $Q_2$, and $Q_3$ to denote the false negative probability for (i) each infected family in the first stage; (ii) each infected member in group testing of the second stage; (iii) each infected member in individual testing of the second stage, respectively. 
%We use the following notation. 
%\begin{align}
%Q &= \Pr(FN|\text{no community}) \nonumber \\
%Q_1 &=\Pr(FN|\text{Family testing}) \nonumber \\
%Q_2 &= \Pr(FN|\text{Testing non-infected families}) \nonumber \\
%Q_3 &= \Pr(FN|\text{Testing infected families})
%\end{align}

Now, we compare $Q$ against the FN probability for the two-stage algorithm, which can be calculated as
$\Pr(FN|\text{Two-stage}) = Q_1Q_2+(1-Q_1)Q_3.$
Consider the case where $k_m\approx M$, \emph{i.e.,} almost all members of an infected family are infected;  we can then choose to  label all members of potentially infected families as infected (effectively by choosing the threshold decoding parameter in~\eqref{Constant-threshold-decision-rule} as  $\delta=\frac{1}{z}-1$). 
In such a case, $Q_3=0$ at the cost of a slight  increase in false positive probability. 
The FN analysis in \eqref{eq:lem:FN-CW} shows that 
\begin{align}
Q \leq \exp{\left[-2\frac{\nTests}{\nDefFamilies \nDefMembersSymmetric}(\znoiseProb\delta)^2\right]}, \;\; 
Q_1\leq \exp{\left[-2\frac{\nTests_1}{\nDefFamilies}(\znoiseProb\delta)^2\right]}. %\nonumber \\
%Q_2&\leq \exp{\left[-2\frac{\nTests_2}{\nDefFamilies Q_1\nDefMembersSymmetric}(\znoiseProb\delta)^2\right]},
\end{align}
Therefore, the FN probability of the two-stage algorithm is:
\begin{align}
\Pr(FN|\text{Two-stage})&\approx  Q_1Q_2\leq Q_1 \leq  e^{-2\frac{\nTests_1}{\nDefFamilies}(\znoiseProb\delta)^2}  \nonumber \\
&=(e^{-2\frac{\nTests}{\nDefFamilies\nDefMembersSymmetric}(\znoiseProb\delta)^2})^{\frac{\nTests_1 \nDefMembersSymmetric}{\nTests}},
\end{align}
which suggests that for $\nTests_1=\alpha\nTests$ with $\alpha$ a constant, the upper bound for $\Pr(\text{FN}|\text{Two-stage})$ can be exponentially smaller than the upper bound for $Q$. 
%$Q=\Pr(\text{FN}|\text{no community})$.



==> Makefile <==
##########################################################
#
# Makefile for LaTeX docs
#
# $Id: 
#

all: pdf

view: 
	open $(PAPER).pdf


PAPER=main

dvi: $(PAPER).dvi 
ps:  $(PAPER).ps 
pdf: $(PAPER).pdf

$(PAPER).pdf:
	pdflatex -jobname=$(PAPER) "\def\flagpaper{}\input{$(PAPER)}"
	bibtex $(PAPER)
	pdflatex -jobname=$(PAPER) "\def\flagpaper{}\input{$(PAPER)}"
	pdflatex -jobname=$(PAPER) "\def\flagpaper{}\input{$(PAPER)}"
	#pstopdf $<	
	#ps2pdf14 -dPDFSETTINGS=/prepress -dEmbedAllFonts=true $*.ps $*.pdf
	$(RM) $(PAPER).dvi *.aux *.log *.blg *.toc *.bbl *.out $(PAPER).ps
	

$(PAPER).dvi: $(wildcard *.tex) $(wildcard *.bib)
	latex -jobname=$(PAPER) "\def\flagpaper{}\input{$(PAPER)}"
	bibtex $(PAPER)
	latex -jobname=$(PAPER) "\def\flagpaper{}\input{$(PAPER)}"
	latex -jobname=$(PAPER) "\def\flagpaper{}\input{$(PAPER)}"
	$(RM) *.aux *.log *.blg *.toc

# only need -Ppdf if using CM fonts
$(PAPER).ps: $(PAPER).dvi
	dvips -e 0 -Ppdf -G0 -tletter -o $@ $<


tarball: $(PAPER).tgz

$(PAPER).tgz: pdf
	tar czvf $@ ./$(PAPER).tex ./$(PAPER).bib ./Makefile ./$(PAPER).pdf

clean:
	$(RM) *.aux *.log *.blg *.bbl *~ *.out *.dvi $(PAPER).pdf *.thm $(PAPER).ps *.synctex.gz 


==> noisy.tex <==

%============================================
\section{Testing with noise}\label{sec:Noisy-Testing}
%\textcolor{cyan}{X: This will be 1.5 pages}\\
%======================================================
Leveraging community structure can improve the reliability when the test outputs are noisy. 
We briefly discuss this point here and provide numerical evidence in ~\Cref{section-experiments}.

{\bf Testing reliability.}
Suppose that noisy tests are used, 
and positive outputs may flip with probability $\znoiseProb$ (Fig.~\ref{fig_Zchannel}). 
To improve testing reliability, we need to add redundancy (extra tests). 
We explore two ways to do so: 
(a) \textit{Repetition testing}, 
where each individual test is repeated $\ell$ times;
this requires a large number of tests, hence is not efficient (a result already known from coding theory). 
%Assuming the decoding rule in \cref{eq:RepTestCond} that uses a parameter $\delta$, we get that
%\begin{equation}
%\Pr(\text{FN}|\text{Repeat each item $\ell$ times}) \leq e^{-2\ell(\znoiseProb\delta)^2}= e^{-2\frac{T}{n}(\znoiseProb\delta)^2}.
%\end{equation}  
%But, it is  that repetition is not very efficient as it requires a large number of repetitions to achieve a low error rate.
(b) \textit{Group testing}, 
where each group test is viewed as a form of coding, 
aiming to introduce redundancy to correct errors.
%We examined 2 commonly used classes of test matrices $\testmatrix$ in this regard: 
%\textit{Bernoulli designs} (akin to binary random coding),
%where each member is included in each test i.i.d. at random with probability $\bernoulliProb$, 
In this regard, one may use \textit{Bernoulli} designs (akin to binary random coding) or \textit{constant column weight} designs for test matrix $\testmatrix$ (akin to constant weight random coding)~\cite{GroupTestingMonograph}.

%Let $\testmatrixEntry_{t,i}$  denote the  $(t,i)$ entry of $\testmatrix$, then:\\
%\noindent $\triangleright$ \textbf{Bernoulli design:} each item is included in each test i.i.d. at random with probability $\bernoulliProb$.\\
%, i.e.
%	\begin{equation}
%	\Pr(\testmatrixEntry_{t,i}=1)=\bernoulliProb, \forall~i\in\{1,2,\cdots,n\}, t\in \{1,2,\cdots,T\}.   
%	\end{equation}
%\noindent $\triangleright$ \textbf{Constant weight design:} each item is included in $\constantWeight$ tests, chosen uniformly at random.

%thus
% $\testmatrix$ has independent columns of constant weight. \\
%For the decision rule in \eqref{Bernoulli-threshold-decision-rule} that uses a parameter $\delta$, we get that  
%\begin{align}
%\Pr(\text{FN}|\text{Bernoulli}) &\leq \left(1-\bernoulliProb+\bernoulliProb e^{-2(\znoiseProb\delta)^2}\right)^{\nTests}, \nonumber \\
%\Pr(\text{FN}|\text{Constant}) &\leq %e^{-2\constantWeight(\znoiseProb\delta)^2}.
%\end{align}


{\bf Community structure.}
To incorporate the community structure, 
we adapt the two-stage algorithm developed in  \Cref{section-two-stage}: 
In the first stage \eqref{step4}, 
we use a test matrix similar to $\testmatrix_1$ from \Cref{sec:nonadapt} to identify all \text{(non-)infected} families. 
For the second stage \eqref{step13}, 
we use a constant-column-weight test design
%\footnote{A similar analysis is possible for adaptations of other noise-free (or noiseless) algorithms to the testing with noise model, and also exploring more redundancy mechanisms for this case.} 
with $\constantWeight=\frac{\nTests}{\nDef}$ and a threshold decoding rule,
where a member is identified as infected (resp. non-infected) if the number of positive (resp. negative) tests it participates in is larger than some threshold.
The following lemma compares the above two-stage algorithm that leverages the community structure against a group testing scheme that uses a traditional constant-column-weight test matrix and a similar threshold-decoding rule but does not take into account the community structure.

\begin{lemma}\label{lemma-exponential-FNprob-noisy}
If tests are noisy following the Z-channel of Fig.~\ref{fig_Zchannel},
a two-stage test design that leverages the community structure has FN probability that is exponentially smaller than that of traditional group testing. 
\end{lemma}


